A Snapshot of the Frontiers of Client Selection in Federated Learning

Federated learning (FL) has been proposed as a privacy-preserving approach in distributed machine learning. A federated learning architecture consists of a central server and a number of clients that have access to private, potentially sensitive data. Clients are able to keep their data in their local machines and only share their locally trained model's parameters with a central server that manages the collaborative learning process. FL has delivered promising results in real-life scenarios, such as healthcare, energy, and finance. However, when the number of participating clients is large, the overhead of managing the clients slows down the learning. Thus, client selection has been introduced as a strategy to limit the number of communicating parties at every step of the process. Since the early na\"{i}ve random selection of clients, several client selection methods have been proposed in the literature. Unfortunately, given that this is an emergent field, there is a lack of a taxonomy of client selection methods, making it hard to compare approaches. In this paper, we propose a taxonomy of client selection in Federated Learning that enables us to shed light on current progress in the field and identify potential areas of future research in this promising area of machine learning.

==> review_answers.tex <==
\subsection{Reviewer Tz1r}
We want to thank the review for agreeing on the positive impact of our paper in future research/engineering directions. We agree with the proposed suggestions and we changed the paper to highlight the importance of the privacy-efficiency trade-off and the attack against the selection strategy. These are missing in past works and it is important to be addressed in future works.
\subsubsection{Privacy Definition and Privacy Loss Definition}
Added paragraphs in introduction and Shared information section (3.4) to highligh the importance of the privacy-efficiency trade-off in client selection.
\subsubsection{Limitations with other FL techniques}
We thank the reviewer to highlight this limitation. It supports the necessity of the shared message section in our taxonomy. Indeed, many of the proposed algorithms are not compatible and it is important to show it when someone propose a new method, following our taxonomy. A possibility to use  SA and LDP is to apply them on the model weights, but send the additional metadata visible to the server. It is not compatible with methods using server side validation, but ones, like \gls{fedcs} can be still used. Added discussion in Section 3.4
\subsubsection{Trustworthiness}
Added paragraph at Section 3.1.1 Resilience to include the attack on client selection.
\subsubsection{Datasets}
Added sentences in page 16 to highlight suggestions.

\subsection{Reviewer wdU1}
\subsubsection{Client selection vs Generic FL problems}
We think that the main disagreement here is that the reviewer views client selection strictly as methods to reduce the number of clients doing the actual training. We tried to be more exclusive for any client participation management strategies. We think that they are all important to capture the big picture. Regarding the methods in Table 1 (and 2), we are unsure of what methods does the review refer to. In case of the ones with weight value interpretation - where the client has to participate in every training round, we would like to point to L1 regularization widely accepted as a feature selection technique. Similarly, these methods can reduce the weight of clients, as far as to zero.
\subsubsection{Which client selection methods are generally good empirically remains unanswered}
Some methods, like pow/d, k-FED, AFL\textsubscript{G} reports efficiency gain compared to random selection. We included these results when we discuss the methods in the paper.
\subsubsection{Figure 1}
Added $\gamma$ function to the figure and text to showcase stateful  servers. Now it is a more general client selection diagram.
\subsubsection{Furthermore}
???
\subsubsection{Section 3.1.1}
Changed limited complexity to limited local training complexity to show that these are restrictions on every clients while training efficiency is the most straightforward motivation to do client selection. Moved FLAME to limited local training complexity.
\subsubsection{Sections 3.1.2}
???
\subsubsection{Section 3.1.3}
idk, I would leave it like this and argue why incentives is a motivation
\subsubsection{Future work after Section 3.1.3}
We extended discussion about privacy following Reviewer Tz1r's suggestion. Maybe find something to support this line of future work?
\subsubsection{In terms of reliability}
I have to check the references!!
\subsubsection{The last two paragraphs of Section 3.1}
idk, just ignore it?
\subsubsection{Section 3.2: (a)} 
Should we remove them?
\subsubsection{Section 3.2: (b)} 
in client selection with privacy budget, the clients stop at different time. If the privacy budget is defined by training rounds, indeed, it means that every client has a fixed number of training round participation. But it is still different than global fixed round termination.
\subsubsection{Section 3.3}
I have to check the references!!
\subsubsection{Section 3.5}
I would ignore this.
\subsubsection{Section 4}
I would ignore this.
